The Third International Verification of Neural Networks Competition (VNN-COMP 2022): Summary and Results

This report summarizes the 3rd International Verification of Neural Networks Competition (VNN-COMP 2022), held as a part of the 5th Workshop on Formal Methods for ML-Enabled Autonomous Systems (FoMLAS), which was collocated with the 34th International Conference on Computer-Aided Verification (CAV). VNN-COMP is held annually to facilitate the fair and objective comparison of state-of-the-art neural network verification tools, encourage the standardization of tool interfaces, and bring together the neural network verification community. To this end, standardized formats for networks (ONNX) and specification (VNN-LIB) were defined, tools were evaluated on equal-cost hardware (using an automatic evaluation pipeline based on AWS instances), and tool parameters were chosen by the participants before the final test sets were made public. In the 2022 iteration, 11 teams participated on a diverse set of 12 scored benchmarks. This report summarizes the rules, benchmarks, participating tools, results, and lessons learned from this iteration of this competition.

==> results2020/results_acasxu_all.tex <==
\subsubsection{ACASXU-ALL}

\begin{figure}[htb]
\centering
\includegraphics[width=0.99\textwidth]{figure/acasxu-all}
\caption{ACASXU-ALL Cactus Plot.}
\label{fig:acasxu_all}
\end{figure}

% the advantage of making tables this way is that each tool defines a single data file for one column of data
% just make sure the results are consistent, use - if tool does not succeed within the timeout

% load table data from files
\pgfplotstableread{data/acasxu-all-front.txt}\dataAcasAll

% load results column and combine with data
\pgfplotstableread{data/acasxu-all-results.txt}\dataAcasAllResults
\pgfplotstablecreatecol[copy column from table={\dataAcasAllResults}{[index] 0}] {results} {\dataAcasAll}

% single column from each tool - make sure to give unique names
\pgfplotstableread{data/acasxu-all-nnenum.txt}\dataAcasAllNnenum
\pgfplotstablecreatecol[copy column from table={\dataAcasAllNnenum}{[index] 0}] {nnenum} {\dataAcasAll}

\pgfplotstableread{data/acasxu-all-NNV.txt}\dataAcasAllNNV
\pgfplotstablecreatecol[copy column from table={\dataAcasAllNNV}{[index] 0}] {NNV} {\dataAcasAll}
\pgfplotstableread{data/acasxu-all-PeregriNN.txt}\dataAcasAllPeregriNN
\pgfplotstablecreatecol[copy column from table={\dataAcasAllPeregriNN}{[index] 0}] {PeregriNN} {\dataAcasAll}
\pgfplotstableread{data/acasxu-all-MIPVerify.txt}\dataAcasAllMIPVerify
\pgfplotstablecreatecol[copy column from table={\dataAcasAllMIPVerify}{[index] 0}] {MIPVerify} {\dataAcasAll}
\pgfplotstableread{data/acasxu-all-venus.txt}\dataAcasAllVenus
\pgfplotstablecreatecol[copy column from table={\dataAcasAllVenus}{[index] 0}] {Venus} {\dataAcasAll}

\pgfplotstableread{data/acasxu-all-eran.txt}\dataAcasAllERAN
\pgfplotstablecreatecol[copy column from table={\dataAcasAllERAN}{[index] 0}] {ERAN} {\dataAcasAll}

% add your tool to the appropriate column header
\providecommand{\myheaders}{\textbf{Prop} & \textbf{Net} & \textbf{Result~~~} & \textbf{nnenum} & \textbf{NNV} & \textbf{PeregriNN} & \textbf{MIPVerify} & \textbf{Venus} & \textbf{ERAN}}

\begin{center}
  \setlength{\tabcolsep}{2pt}
\pgfplotstabletypeset[
    empty header,
    begin table=\begin{longtable},
    column type/.add={r},
    display columns/0/.style={column type = {c}},
    display columns/1/.style={column type = {l}},
    display columns/2/.style={string type, column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/3/.style={column type = {r}},
    display columns/4/.style={column type = {r}},
    display columns/5/.style={column type = {r}},
    display columns/6/.style={column type = {r}},
    display columns/7/.style={column type = {r}},
    every first row/.append style={before row={%
    \caption{Tool Runtime (sec) for ACASXU-ALL.}%
    \label{tab:acasxuAllTable}\\\toprule
    \myheaders
    %\textbf{Prop} & \textbf{Net}
    \\ \toprule    
    \endfirsthead
    \multicolumn{4}{l}%
    {{\bfseries Table \thetable\ Continued}}
    \\
    \toprule 
    %%
    \myheaders
    \\ \toprule 
    \endhead
    %
    \midrule
    %\midrule \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
    \endfoot
    %
    %\midrule
    %\multicolumn{2}{r}{{Concluded}}
    \bottomrule
    \endlastfoot
    }},%
    %
    end table=\end{longtable},
    col sep=comma,
    string type,
    ]{\dataAcasAll}
\end{center}

==> results2020/results_acasxu_hard.tex <==
\subsubsection{ACASXU-HARD}

% the advantage of making tables this way is that each tool defines a single data file for one column of data
% just make sure the results are consistent, use - if tool does not succeed within the timeout

% load table data from files
\pgfplotstableread{data/acasxu-hard-front.txt}\dataAcasHard


% load results column and combine with data
\pgfplotstableread{data/acasxu-hard-results.txt}\dataAcasHardResults
\pgfplotstablecreatecol[copy column from table={\dataAcasHardResults}{[index] 0}] {results} {\dataAcasHard}

% single column from each tool - make sure to give unique names
\pgfplotstableread{data/acasxu-hard-nnenum.txt}\dataAcasHardNnenum
\pgfplotstablecreatecol[copy column from table={\dataAcasHardNnenum}{[index] 0}] {nnenum} {\dataAcasHard}

\pgfplotstableread{data/acasxu-hard-NNV.txt}\dataAcasHardNNV
\pgfplotstablecreatecol[copy column from table={\dataAcasHardNNV}{[index] 0}] {NNV} {\dataAcasHard}

\pgfplotstableread{data/acasxu-hard-PeregriNN.txt}\dataAcasHardPeregriNN
\pgfplotstablecreatecol[copy column from table={\dataAcasHardPeregriNN}{[index] 0}] {PeregriNN} {\dataAcasHard}

\pgfplotstableread{data/acasxu-hard-MIPVerify.txt}\dataAcasHardMIPVerify
\pgfplotstablecreatecol[copy column from table={\dataAcasHardMIPVerify}{[index] 0}] {MIPVerify} {\dataAcasHard}

\pgfplotstableread{data/acasxu-hard-venus.txt}\dataAcasHardVenus
\pgfplotstablecreatecol[copy column from table={\dataAcasHardVenus}{[index] 0}] {Venus} {\dataAcasHard}

\pgfplotstableread{data/acasxu-hard-eran.txt}\dataAcasHardERAN
\pgfplotstablecreatecol[copy column from table={\dataAcasHardERAN}{[index] 0}] {ERAN} {\dataAcasHard}

% add your tool to the appropriate column header
\renewcommand{\myheaders}{\textbf{Prop} & \textbf{Net} & \textbf{Result~~~} & \textbf{nnenum} & \textbf{NNV} & \textbf{PeregriNN} & \textbf{MIPVerify} & \textbf{Venus} & \textbf{ERAN}}

\newpage

\begin{center}
  \setlength{\tabcolsep}{2pt}
\pgfplotstabletypeset[
    empty header,
    begin table=\begin{longtable},
    column type/.add={r},
    display columns/0/.style={column type = {c}},
    display columns/1/.style={column type = {l}},
    display columns/2/.style={string type, column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/3/.style={column type = {r}},
    display columns/4/.style={column type = {r}},
    display columns/5/.style={column type = {r}},
    display columns/6/.style={column type = {r}},
    display columns/7/.style={column type = {r}},
    every first row/.append style={before row={%
    \caption{Tool Runtime (sec) for ACASXU-HARD.}%
    \label{tab:acasxuHardTable}\\\toprule
    \myheaders
    %\textbf{Prop} & \textbf{Net}
    \\ \toprule    
    \endfirsthead
    \multicolumn{4}{l}%
    {{\bfseries Table \thetable\ Continued}}
    \\
    \toprule 
    %%
    \myheaders
    \\ \toprule 
    \endhead
    %
    \midrule
    %\midrule \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
    \endfoot
    %
    %\midrule
    %\multicolumn{2}{r}{{Concluded}}
    \bottomrule
    \endlastfoot
    }},%
    %
    end table=\end{longtable},
    col sep=comma,
    string type,
    ]{\dataAcasHard}
\end{center}

==> results2020/results_ggn_cnn.tex <==
\subsubsection{GGN - Convolutional Networks}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\textwidth]{figure/ggn-cnn}
\caption{GGN-CNN Cactus Plot.}
\label{fig:ggn_cnn}
\end{figure}

% the advantage of making tables this way is that each tool defines a single data file for one column of data
% just make sure the results are consistent, use - if tool does not succeed within the timeout

% load table data from files
\pgfplotstableread{data/ggn-all-front.txt}\dataGgnAll


% load results column and combine with data
\pgfplotstableread{data/ggn-all-results.txt}\dataGgnAllResults
\pgfplotstablecreatecol[copy column from table={\dataGgnAllResults}{[index] 0}] {results} {\dataGgnAll}

% single column from each tool - make sure to give unique names
\pgfplotstableread{data/ggn-all-nnenum.txt}\dataGgnAllNnenum
\pgfplotstablecreatecol[copy column from table={\dataGgnAllNnenum}{[index] 0}] {nnenum} {\dataGgnAll}

\pgfplotstableread{data/ggn-all-NNV.txt}\dataGgnAllNNV
\pgfplotstablecreatecol[copy column from table={\dataGgnAllNNV}{[index] 0}] {NNV} {\dataGgnAll}

\pgfplotstableread{data/ggn-all-verinet.txt}\dataGgnAllVeriNet
\pgfplotstablecreatecol[copy column from table={\dataGgnAllVeriNet}{[index] 0}] {VeriNet} {\dataGgnAll}

\pgfplotstableread{data/ggn-all-MIPVerify.txt}\dataGgnAllMIPVerify
\pgfplotstablecreatecol[copy column from table={\dataGgnAllMIPVerify}{[index] 0}] {MIPVerify} {\dataGgnAll}

\pgfplotstableread{data/ggn-all-oval.txt}\dataGgnAllOval
\pgfplotstablecreatecol[copy column from table={\dataGgnAllOval}{[index] 0}] {Oval} {\dataGgnAll}

\pgfplotstableread{data/ggn-all-eran.txt}\dataGgnAllERAN
\pgfplotstablecreatecol[copy column from table={\dataGgnAllERAN}{[index] 0}] {unique_name5} {\dataGgnAll}

% add your tool to the appropriate column header
\renewcommand{\myheaders}{\textbf{Net} & \textbf{Ep} & \textbf{Image} & \textbf{Result~~~} & \textbf{nnenum} & \textbf{NNV} & \textbf{VeriNet} & \textbf{MIPVerify} & \textbf{Oval} & \textbf{ERAN}}

\begin{center}
  \setlength{\tabcolsep}{2pt}
\pgfplotstabletypeset[
    empty header,
    begin table=\begin{longtable},
    column type/.add={r},
    display columns/0/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/1/.style={column type = {l}},
    display columns/2/.style={column type = {c}},
    display columns/3/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/4/.style={column type = {r}},
    display columns/5/.style={column type = {r}},
    display columns/6/.style={column type = {r}},
    display columns/7/.style={column type = {r}},
    display columns/8/.style={column type = {r}},
    every first row/.append style={before row={%
    \caption{Tool Runtime (sec) for GGN-CNN.}%
    \label{tab:ggnAllTable}\\\toprule
    \myheaders
    %\textbf{Prop} & \textbf{Net}
    \\ \toprule    
    \endfirsthead
    \multicolumn{4}{l}%
    {{\bfseries Table \thetable\ Continued}}
    \\
    \toprule 
    %%
    \myheaders
    \\ \toprule 
    \endhead
    %
    \midrule
    %\midrule \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
    \endfoot
    %
    %\midrule
    %\multicolumn{2}{r}{{Concluded}}
    \bottomrule
    \endlastfoot
    }},%
    %
    end table=\end{longtable},
    col sep=comma,
    string type,
    ]{\dataGgnAll}
\end{center}

==> results2020/results_neel_fcn.tex <==
\subsubsection{NEEL - Nonlinear Networks}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\textwidth]{figure/neel-nln}
\caption{NEEL-NLN Cactus Plot.}
\label{fig:neel_nln}
\end{figure}

% the advantage of making tables this way is that each tool defines a single data file for one column of data
% just make sure the results are consistent, use - if tool does not succeed within the timeout

% load table data from files
\pgfplotstableread{data/neel-all-front.txt}\dataneelAll


% load results column and combine with data
\pgfplotstableread{data/neel-all-results.txt}\dataneelAllResults
\pgfplotstablecreatecol[copy column from table={\dataneelAllResults}{[index] 0}] {results} {\dataneelAll}

% single column from each tool - make sure to give unique names
\pgfplotstableread{data/neel-all-NNV.txt}\dataneelAllNNV
\pgfplotstablecreatecol[copy column from table={\dataneelAllNNV}{[index] 0}] {NNV} {\dataneelAll}

\pgfplotstableread{data/neel-all-verinet.txt}\dataneelAllVeriNet
\pgfplotstablecreatecol[copy column from table={\dataneelAllVeriNet}{[index] 0}] {VeriNet} {\dataneelAll}

\pgfplotstableread{data/neel-all-eran.txt}\dataneelAllERAN
\pgfplotstablecreatecol[copy column from table={\dataneelAllERAN}{[index] 0}] {ERAN} {\dataneelAll}
%\pgfplotstablecreatecol[copy column from table={\dataneelAllEmpty}{[index] 0}] {unique_name5} {\dataneelAll}

% add your tool to the appropriate column header
\renewcommand{\myheaders}{\textbf{Net} & \textbf{Ep} & \textbf{Image} & \textbf{Result~~~} & \textbf{NNV} & \textbf{VeriNet} & \textbf{ERAN}}

\begin{center}
  \setlength{\tabcolsep}{2pt}
\pgfplotstabletypeset[
    empty header,
    begin table=\begin{longtable},
    column type/.add={r},
    display columns/0/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/1/.style={column type = {l}},
    display columns/2/.style={column type = {c}},
    every row 8 column 3/.style={column type = {l}, postproc cell content/.style={
          @cell content=\textcolor{red}{\texttt{##1}}
        }},
    display columns/3/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/4/.style={column type = {r}},
    display columns/5/.style={column type = {r}},
    every first row/.append style={before row={%
    \caption{Tool Runtime (sec) for NEEL-NLN.}%
    \label{tab:neelAllTable}\\\toprule
    \myheaders
    %\textbf{Prop} & \textbf{Net}
    \\ \toprule    
    \endfirsthead
    \multicolumn{4}{l}%
    {{\bfseries Table \thetable\ Continued}}
    \\
    \toprule 
    %%
    \myheaders
    \\ \toprule 
    \endhead
    %
    \midrule
    %\midrule \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
    \endfoot
    %
    %\midrule
    %\multicolumn{2}{r}{{Concluded}}
    \bottomrule
    \endlastfoot
    }},%
    %
    end table=\end{longtable},
    col sep=comma,
    string type,
    ]{\dataneelAll}
\end{center}

==> results2020/results_oval_cnn.tex <==
\newpage
\subsubsection{OVAL - Convolutional Networks}

\begin{figure}[htb]
\centering
 \includegraphics[width=0.9\textwidth]{figure/oval-cnn}
\caption{OVAL-CNN Cactus Plot.}
 \label{fig:oval_cnn}
 \end{figure}

% the advantage of making tables this way is that each tool defines a single data file for one column of data
% just make sure the results are consistent, use - if tool does not succeed within the timeout

% load table data from files
\pgfplotstableread{data/oval-dataset-front.txt}\dataOvalAll

% load results column and combine with data
\pgfplotstableread{data/oval-dataset-results.txt}\dataOvalAllResults
\pgfplotstablecreatecol[copy column from table={\dataOvalAllResults}{[index] 0}] {results} {\dataOvalAll}

% single column from each tool - make sure to give unique names
\pgfplotstableread{data/oval-dataset-oval.txt}\dataOvalAllNnenum
\pgfplotstablecreatecol[copy column from table={\dataOvalAllNnenum}{[index] 0}] {oval} {\dataOvalAll}

\pgfplotstableread{data/oval-dataset-eran.txt}\dataOvalAllERAN
\pgfplotstablecreatecol[copy column from table={\dataOvalAllERAN}{[index] 0}] {ERAN} {\dataOvalAll}

% add your tool to the appropriate column header
\renewcommand{\myheaders}{\textbf{Net~~} & \textbf{Image} & \textbf{Ep~~~} & \textbf{Result~~~} & \textbf{Oval} & \textbf{ERAN}}

\begin{center}
  \setlength{\tabcolsep}{2pt}
\pgfplotstabletypeset[
    empty header,
    begin table=\begin{longtable},
    column type/.add={r},
    display columns/0/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/1/.style={column type = {r}},
    display columns/2/.style={column type = {c}},
    display columns/3/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/4/.style={column type = {r}},
    display columns/5/.style={column type = {r}},
    display columns/6/.style={column type = {r}},
    display columns/7/.style={column type = {r}},
    display columns/8/.style={column type = {r}},
    every first row/.append style={before row={%
    \caption{Tool Runtime (sec) for OVAL-CNN.}%
    \label{tab:ovalAllTable}\\\toprule
    \myheaders
    %\textbf{Prop} & \textbf{Net}
    \\ \toprule    
    \endfirsthead
    \multicolumn{4}{l}%
    {{\bfseries Table \thetable\ Continued}}
    \\
    \toprule 
    %%
    \myheaders
    \\ \toprule 
    \endhead
    %
    \midrule
    %\midrule \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
    \endfoot
    %
    %\midrule
    %\multicolumn{2}{r}{{Concluded}}
    \bottomrule
    \endlastfoot
    }},%
    %
    end table=\end{longtable},
    col sep=comma,
    string type,
    ]{\dataOvalAll}
\end{center}

==> results2020/results_pat_fcn.tex <==
\newpage
\subsubsection{Pat Fully Connected Networks}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\textwidth]{figure/pat-fcn}
\caption{PAT-FCN Cactus Plot.}
\label{fig:pat_fcn}
\end{figure}

% the advantage of making tables this way is that each tool defines a single data file for one column of data
% just make sure the results are consistent, use - if tool does not succeed within the timeout

% load table data from files
\pgfplotstableread{data/pat-all-front.txt}\dataPatAll

% load results column and combine with data
\pgfplotstableread{data/pat-all-results.txt}\dataPatAllResults
\pgfplotstablecreatecol[copy column from table={\dataPatAllResults}{[index] 0}] {results} {\dataPatAll}

% single column from each tool - make sure to give unique names
\pgfplotstableread{data/pat-all-nnenum.txt}\dataPatAllNnenum
\pgfplotstablecreatecol[copy column from table={\dataPatAllNnenum}{[index] 0}] {nnenum} {\dataPatAll}

\pgfplotstableread{data/pat-all-NNV.txt}\dataPatAllNNV
\pgfplotstablecreatecol[copy column from table={\dataPatAllNNV}{[index] 0}] {NNV} {\dataPatAll}

\pgfplotstableread{data/pat-all-PeregriNN.txt}\dataPatAllPeregriNN
\pgfplotstablecreatecol[copy column from table={\dataPatAllPeregriNN}{[index] 0}] {PeregriNN} {\dataPatAll}

\pgfplotstableread{data/pat-all-VeriNet.txt}\dataPatAllVeriNet
\pgfplotstablecreatecol[copy column from table={\dataPatAllVeriNet}{[index] 0}] {VeriNet} {\dataPatAll}

\pgfplotstableread{data/pat-all-MIPVerify.txt}\dataPatAllMIPVerify
\pgfplotstablecreatecol[copy column from table={\dataPatAllMIPVerify}{[index] 0}] {MIPVerify} {\dataPatAll} 

\pgfplotstableread{data/pat-all-venus.txt}\dataPatAllVenus
\pgfplotstablecreatecol[copy column from table={\dataPatAllVenus}{[index] 0}] {Venus} {\dataPatAll} 

\pgfplotstableread{data/pat-all-eran.txt}\dataPatAllERAN
\pgfplotstablecreatecol[copy column from table={\dataPatAllERAN}{[index] 0}] {ERAN} {\dataPatAll} 


% add your tool to the appropriate column header
%\renewcommand{\myheaders}{\textbf{Net} & \textbf{Ep} & \textbf{Image} & \textbf{Result~~~} & \textbf{nnenum} & \textbf{NNV} & \textbf{PeregriNN} & \textbf{VeriNet} & \textbf{MIPVerify} & \textbf{Venus} & \textbf{ERAN}}

% shortened names
\renewcommand{\myheaders}{\textbf{Net} & \textbf{Ep} & \textbf{Im} & \textbf{Result} & \textbf{nnenum} & \textbf{NNV} & \textbf{PeregriNN} & \textbf{VeriNet} & \textbf{MIPVerify} & \textbf{Venus} & \textbf{ERAN}}

\begin{center}
  \setlength{\tabcolsep}{2pt}
\pgfplotstabletypeset[
    empty header,
    begin table=\begin{longtable},
    column type/.add={r},
    display columns/0/.style={column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/1/.style={column type = {l}},
    display columns/2/.style={column type = {c}},
    display columns/3/.style={string type, column type = {l}, postproc cell content/.style={
          @cell content=\texttt{##1}
        }},
    display columns/4/.style={column type = {r}},
    display columns/5/.style={column type = {r}},
    display columns/6/.style={column type = {r}},
    display columns/7/.style={column type = {r}},
    display columns/8/.style={column type = {r}},
    display columns/9/.style={column type = {r}},
    every first row/.append style={before row={%
    \caption{Tool Runtime (sec) for PAT-FCN.}%
    \label{tab:patTable}\\\toprule
    \myheaders
    %\textbf{Prop} & \textbf{Net}
    \\ \toprule    
    \endfirsthead
    \multicolumn{4}{l}%
    {{\bfseries Table \thetable\ Continued}}
    \\
    \toprule 
    %%
    \myheaders
    \\ \toprule 
    \endhead
    %
    \midrule
    %\midrule \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
    \endfoot
    %
    %\midrule
    %\multicolumn{2}{r}{{Concluded}}
    \bottomrule
    \endlastfoot
    }},%
    %
    end table=\end{longtable},
    col sep=comma,
    string type,
    ]{\dataPatAll}
\end{center}
